Precise predictions for boosted Higgs production

Inclusive Higgs boson production at large transverse momentum is induced by different production channels. We focus on the leading production through gluon fusion, and perform a consistent combination of the state of the art calculations obtained in the infinite-top-mass effective theory at next-to-next-to-leading order (NNLO) and in the full Standard Model (SM) at next-to-leading order (NLO). We thus present approximate QCD predictions for this process at NNLO, and a study of the corresponding perturbative uncertainties. This calculation is then compared with those obtained with commonly used event generators, and we observe that the description of the considered kinematic regime provided by these tools is in good agreement with state of the art calculations. Finally, we present accurate predictions for other production channels such as vector boson fusion, and associated production with a gauge boson, and with a $t\bar{t}$ pair. We find that, at large transverse momentum, the contribution of other production modes is substantial, and therefore must be included for a precise theory prediction of this observable.

==> Chapters/VBF.tex <==
\section{Predictions from Vector Boson Fusion}
\label{sec:vbf}
We conclude this note by reporting the results for the vector boson
fusion (VBF) contribution to the boosted-Higgs cross section. This is
obtained using the predictions 

of
ref.~\cite{Dreyer:2016oyx,Cacciari:2015jma}, where the VBF cross
section is computed to approximate N$^3$LO accuracy in perturbative
QCD.  Estimated uncertainties due to imprecise knowledge of coupling
constants, parton distribution functions, missing higher perturbative
orders and corrections due to the chosen approximation amount in total
to roughly $3\%$.  Note, that also electro-weak corrections to the
inclusive VBF cross section start to play an important role and are at
the level of $\sim -20 \%$, as discussed in
Appendix~\ref{app:channels}. 

\begin{figure*}[htb]
\centering
\includegraphics[width=.65\textwidth]{figures/VBF_cumulant.pdf}
\caption{Cumulative cross section from vector-boson fusion in the
  boosted regime. The Higgs branching ratio into bottom quarks is included.}
\label{fig:VBF}
\end{figure*}

We observe that the VBF contribution at the relevant $p_\perp$ values
is a significant fraction of the total cross section. We consider its
value at $p_\perp=450$~GeV as a reference value. Using a
$BR(H\to b\bar b)=0.5824$, we obtain the results reported in
Table~\ref{tab:VBFTable}, where we observe that the VBF contribution
accounts for $30\%$ of the total cross section in this region. The
errors indicate only the scale uncertainty. However, as mentioned
above, further sources of uncertainties are present. The cumulative
cross section as a function of $p_\perp$ is reported in
Fig.~\ref{fig:VBF}.  {\renewcommand{\arraystretch}{1.5}
\begin{table*}[htp!]
  \vspace*{0.3ex}
  \begin{center}
\begin{small}
%    \begin{tabular}{ll@{\hspace{12mm}}l@{\hspace{12mm}}l}
    \begin{tabular}{c|c|c|c}
%
$p_\perp^{\rm cut}$& %\phantom{\Huge{X}}
  
   $\Sigma_{\rm ggF}( p_\perp^{\rm cut})\times {\rm BR}$ [fb]& $\Sigma_{\rm VBF}(
                                             p_\perp^{\rm cut})\times {\rm BR}$
                                                 [fb]& $\Sigma_{\rm
                                                       ggF+VBF}(
                                                       p_\perp^{\rm cut})\times {\rm
                                                       BR}$ [fb]\\
\hline
% 
$450~\text{GeV}$    & $10.53^{+8.9\%}_{-11.5\%}$ & $4.71^{+0.14\%}_{-0.14\%}$ &
                                                                       $15.24^{+7.51\%}_{-8.89\%}$
    \end{tabular}
\end{small}
  \end{center}
  \caption{Predictions including the VBF contribution. The
    uncertainties in the gluon fusion cross section are determined by
    combining the various sources in quadrature as described in the
    previous section. The errors in the VBF contribution indicates the
    QCD scale uncertainty.
  }
\label{tab:VBFTable}
\end{table*}
}

It should also be noted that other production modes gain in importance relative to the gluon fusion production mechanism as the transverse momentum of the Higgs boson is increased. 
The final state signature arising from the production of a Higgs boson
in association with a vector
boson~\cite{Gleisberg:2008ta,Cascioli:2011va,Kallweit:2014xda,Schonherr:2017qcj,Luisoni:2013kna}
or a top quark pair~\cite{Gleisberg:2008ta,Cascioli:2011va} is however
significantly different such that we do not include explicit values
for the respective cross sections here. For reference we display the
contributions of the different production modes in Appendix~\ref{app:channels}.

%For reference we display the absolute and relative importance of the different production mechanisms in figure~\ref{fig:prodmodes} respectively.
%
% \begin{figure*}[htb]
%\centering
%\includegraphics[width=.45\textwidth]{figures/13TeV-1.pdf}
%\includegraphics[width=.45\textwidth]{figures/13TeV-ratio-1.pdf}
%\caption{
%Cumulative cross section for the production of a Higgs boson as a function of the lowest Higgs boson transverse momentum. 
%The cross section due to the gluon-fusion (green), VBF (red), vector boson associated (blue) and top-quark pair associated (magenta) production mode are shown in absolute values (left) and relative size (right).
% }
%\label{fig:prodmodes}
%\end{figure*}



\begin{table*}[htp!]
\begin{equation}
\begin{array}{|c|c|c|c|}
\hline
p_\perp^{\rm cut} \text{[GeV]} & \Sigma_{\rm ggF}( p_\perp^{\rm cut}) \text{ [fb]} & \Sigma_{\rm VBF}( p_\perp^{\rm cut})   \text{ [fb]}  &  \Sigma_{\rm ggF+VBF}( p_\perp^{\rm cut})  \text{ [fb]} \\
\hline
400 & 33.30^{10.89 \%}_{-12.91 \%} & 14.26^{20\%}_{-20\%} & 47.56^{9.70\%}_{-10.85\%} \\
 \hline
410 & 29.34^{10.86 \%}_{-12.85 \%} & 12.70^{20\%}_{-20\%} & 42.03^{9.69\%}_{-10.82\%} \\
 \hline
420 & 25.95^{10.78 \%}_{-12.80 \%} & 11.32^{20\%}_{-20\%} & 37.27^{9.66\%}_{-10.79\%} \\
 \hline
430 & 22.97^{10.79 \%}_{-12.80 \%} & 10.10^{20\%}_{-20\%} & 33.08^{9.67\%}_{-10.78\%} \\
 \hline
440 & 20.39^{10.80 \%}_{-12.82 \%} & 9.04^{20\%}_{-20\%} & 29.42^{9.68\%}_{-10.80\%} \\
 \hline
450 & 18.08^{10.78 \%}_{-12.79 \%} & 8.09^{20\%}_{-20\%} & 26.17^{9.68\%}_{-10.78\%} \\
 \hline
460 & 16.01^{10.68 \%}_{-12.74 \%} & 7.26^{20\%}_{-20\%} & 23.28^{9.64\%}_{-10.76\%} \\
 \hline
470 & 14.27^{10.67 \%}_{-12.73 \%} & 6.52^{20\%}_{-20\%} & 20.79^{9.64\%}_{-10.76\%} \\
 \hline
480 & 12.77^{10.76 \%}_{-12.79 \%} & 5.87^{20\%}_{-20\%} & 18.63^{9.70\%}_{-10.79\%} \\
 \hline
490 & 11.39^{10.75 \%}_{-12.76 \%} & 5.29^{20\%}_{-20\%} & 16.68^{9.70\%}_{-10.78\%} \\
 \hline
500 & 10.17^{10.67 \%}_{-12.74 \%} & 4.77^{20\%}_{-20\%} & 14.95^{9.67\%}_{-10.77\%} \\
 \hline
510 & 9.11^{10.69 \%}_{-12.72 \%} & 4.31^{20\%}_{-20\%} & 13.41^{9.69\%}_{-10.76\%} \\
 \hline
520 & 8.15^{10.67 \%}_{-12.70 \%} & 3.90^{20\%}_{-20\%} & 12.05^{9.70\%}_{-10.76\%} \\
 \hline
530 & 7.29^{10.60 \%}_{-12.66 \%} & 3.54^{20\%}_{-20\%} & 10.83^{9.67\%}_{-10.74\%} \\
 \hline
540 & 6.52^{10.50 \%}_{-12.58 \%} & 3.21^{20\%}_{-20\%} & 9.73^{9.65\%}_{-10.70\%} \\
 \hline
550 & 5.87^{10.54 \%}_{-12.60 \%} & 2.91^{20\%}_{-20\%} & 8.79^{9.68\%}_{-10.72\%} \\
 \hline
560 & 5.29^{10.56 \%}_{-12.63 \%} & 2.65^{20\%}_{-20\%} & 7.94^{9.70\%}_{-10.74\%} \\
 \hline
570 & 4.76^{10.47 \%}_{-12.59 \%} & 2.41^{20\%}_{-20\%} & 7.17^{9.67\%}_{-10.73\%} \\
 \hline
580 & 4.29^{10.44 \%}_{-12.58 \%} & 2.20^{20\%}_{-20\%} & 6.48^{9.68\%}_{-10.73\%} \\
 \hline
590 & 3.86^{10.42 \%}_{-12.53 \%} & 2.01^{20\%}_{-20\%} & 5.87^{9.68\%}_{-10.71\%} \\
 \hline
 \end{array}
 \nonumber
\end{equation}
  \caption{Predictions for the cumulative Higgs boson cross section as
    a function of the Higgs boson transverse momentum cut $p_\perp$.
    We show predictions due to the ggF and VBF production mechanism
    and their combination.  The uncertainties of the combined
    prediction are computed by combining the individual uncertainties
    in quadrature.  }
\label{tab:finaltab}
\end{table*}

